A System Parametrization for Direct Data-Driven Analysis and Control with Error-in-Variables

In this paper, we present a new parametrization to perform direct data-driven analysis and controller synthesis for the error-in-variables case. To achieve this, we employ the Sherman-Morrison-Woodbury formula to transform the problem into a linear fractional transformation (LFT) with unknown measurement errors and disturbances as uncertainties. For bounded uncertainties, we apply robust control techniques to derive a guaranteed upper bound on the H2-norm of the unknown true system. To this end, a single semidefinite program (SDP) needs to be solved, with complexity that is independent of the amount of data. Furthermore, we exploit the signal-to-noise ratio to provide a data-dependent condition, that characterizes whether the proposed parametrization can be employed. The modular formulation allows to extend this framework to controller synthesis with different performance criteria, input-output settings, and various system properties. Finally, we validate the proposed approach through a numerical example.

==> sec/figs/ECC_Statistics.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\linewidth,
height=0.75\linewidth,
at={(0\linewidth,0\linewidth)},
scale only axis,
xmin=0,
xmax=300,
xlabel style={font=\color{white!15!black}},
xlabel={N},
ymin=0,
ymax=1.2,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, line width=1.0pt]
  table[row sep=crcr]{%
7	1.01183535716665\\
8	1.00508893291974\\
9	0.68729005591268\\
10	0.624185334026535\\
12	0.662502289697766\\
15	0.431676179984261\\
20	0.186669428940095\\
25	0.097776941992781\\
30	0.0674666554012567\\
40	0.0474472517845954\\
50	0.0433996327169081\\
70	0.0387324999621969\\
100	0.0366431395905191\\
150	0.0343435148112714\\
200	0.0339393104112452\\
300	0.0338033236875188\\
};
\addlegendentry{$\epsilon_{G^\star}$}

\addplot [color=blue, dashed, line width=1.0pt]
  table[row sep=crcr]{%
7	0.2665\\
8	0.5245\\
9	0.69\\
10	0.751\\
12	0.816\\
15	0.892\\
20	0.9815\\
25	0.9945\\
30	0.999\\
40	0.9985\\
50	0.99\\
70	0.991\\
100	0.9805\\
150	0.982\\
200	0.992\\
300	0.9985\\
};
\addlegendentry{success rate $G^\star$}

\addplot [color=red, line width=1.0pt]
  table[row sep=crcr]{%
7	1.01183535775337\\
8	0.935360241978803\\
9	0.605404167744962\\
10	0.681354806693654\\
12	0.326202293889107\\
15	0.233760184635835\\
20	0.294428371756955\\
25	0.187955394189386\\
30	0.157993037493089\\
40	0.1132135823597\\
50	0.0986157382765081\\
70	0.0718983596230663\\
100	0.0605457060828005\\
150	0.0458365562628748\\
200	0.042572578192703\\
300	0.0373581938815611\\
};
\addlegendentry{$\epsilon_{G^\dagger}$}

\addplot [color=red, dashed, line width=1.0pt]
  table[row sep=crcr]{%
7	0.2665\\
8	0.5265\\
9	0.7295\\
10	0.842\\
12	0.927\\
15	0.969\\
20	0.9815\\
25	0.9865\\
30	0.9935\\
40	0.9965\\
50	0.999\\
70	0.9995\\
100	1\\
150	1\\
200	1\\
300	1\\
};
\addlegendentry{success rate $G^\dagger$}

\end{axis}

\begin{axis}[%
width=0.245\linewidth,
height=0.322\linewidth,
at={(0.675\linewidth,0.083\linewidth)},
scale only axis,
xmin=7,
xmax=30,
ymin=0,
ymax=1.2,
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
xmajorgrids,
ymajorgrids
]
\addplot [color=blue, line width=0.8pt, forget plot]
  table[row sep=crcr]{%
7	1.01183535716665\\
8	1.00508893291974\\
9	0.68729005591268\\
10	0.624185334026535\\
12	0.662502289697766\\
15	0.431676179984261\\
20	0.186669428940095\\
25	0.097776941992781\\
30	0.0674666554012567\\
};
\addplot [color=blue, dashed, line width=0.8pt, forget plot]
  table[row sep=crcr]{%
7	0.2665\\
8	0.5245\\
9	0.69\\
10	0.751\\
12	0.816\\
15	0.892\\
20	0.9815\\
25	0.9945\\
30	0.999\\
};
\addplot [color=red, line width=0.8pt, forget plot]
  table[row sep=crcr]{%
7	1.01183535775337\\
8	0.935360241978803\\
9	0.605404167744962\\
10	0.681354806693654\\
12	0.326202293889107\\
15	0.233760184635835\\
20	0.294428371756955\\
25	0.187955394189386\\
30	0.157993037493089\\
};
\addplot [color=red, dashed, line width=0.8pt, forget plot]
  table[row sep=crcr]{%
7	0.2665\\
8	0.5265\\
9	0.7295\\
10	0.842\\
12	0.927\\
15	0.969\\
20	0.9815\\
25	0.9865\\
30	0.9935\\
};
\end{axis}
\end{tikzpicture}%
